Differentiable Bandit Exploration

Exploration policies in Bayesian bandits maximize the average reward over problem instances drawn from some distribution $\mathcal{P}$. In this work, we learn such policies for an unknown distribution $\mathcal{P}$ using samples from $\mathcal{P}$. Our approach is a form of meta-learning and exploits properties of $\mathcal{P}$ without making strong assumptions about its form. To do this, we parameterize our policies in a differentiable way and optimize them by policy gradients, an approach that is general and easy to implement. We derive effective gradient estimators and introduce novel variance reduction techniques. We also analyze and experiment with various bandit policy classes, including neural networks and a novel softmax policy. The latter has regret guarantees and is a natural starting point for our optimization. Our experiments show the versatility of our approach. We also observe that neural network policies can learn implicit biases expressed only through the sampled instances.

==> BroaderImpact.tex <==
%!TEX root = Paper.tex

\section*{Broader Impact}
\label{sec:broader impact}

We develop bandit-style exploration algorithms that can be easily trained on historical data. This fundamentally alters the current prevalent approach to bandit algorithm design, which is by theory. Bandit algorithms are often deployed in user-facing domains. However, we do not propose any new domain. Therefore, our impact on users should be limited to the domains that already exist. Beyond this, we are not aware of any foreseeable societal consequences of our work, such as on welfare, fairness, privacy, and so on.

